CNM: An Interpretable Complex-valued Network for Matching

This paper seeks to model human language by the mathematical framework of quantum physics. With the well-designed mathematical formulations in quantum physics, this framework unifies different linguistic units in a single complex-valued vector space, e.g. words as particles in quantum states and sentences as mixed systems. A complex-valued network is built to implement this framework for semantic matching. With well-constrained complex-valued components, the network admits interpretations to explicit physical meanings. The proposed complex-valued network for matching (CNM) achieves comparable performances to strong CNN and RNN baselines on two benchmarking question answering (QA) datasets.

==> related_work.tex <==
\vspace{-5pt}
\section{Related Works}


\subsection{Question Answering}
To be added.


% As a mainstream sentence modeling approach, sentence embedding mainly models a sentence as a fix-length vector to represent its semantics. It can be achieved through unsupervised~\cite{pagliardini_unsupervised_2017,Kiros:2015:SV:2969442.2969607,hill_learning_2016_a}, supervised~\cite{bansal_towards_2016,arora_simple_2016} approaches or by advanced deep neural networks~\cite{tang_document_2015,kim_convolutional_2014}. Essentially, these works leverage low-level co-occurrences or sequential orders as the basis of word semantic features, and apply highly linear operations to word features in order to obtain a sentence representation. Even though they have achieved superior performances in many NLP tasks, they are insufficient to model the more complicated non-linear semantic combination of words as described above.
 

% , which tries to use Quantum Theory to re-formalize information retrieval in a sound unified framework for manipulating vector spaces and probability,
\subsection{Quantum Theory in Information Retrieval}
Ever since the pioneering work of Van Rijsbergen~\cite{van2004geometry} and Melucci~\cite{melucci2008basis}, Quantum Theory has been applied in Information Retrieval, yielding a series of novel retrieval models, such as quantum probability ranking principle~\cite{pothos2009quantum,zuccon2010using} and quantum language model~\cite{sordoni2013modeling}. However, these research are limited to ad-hoc retrieval scenarios and fail to address more complicated tasks in information access and retrieval (IAR), which requires fine-grained modeling of textual data. In such scenarios as text classification, question answering, reading comprehension and multi-turn dialogue systems, embedding-based neural networks are the state of art. The first quantum-inspired model specifically aiming at these tasks is a Neural Network based Quantum-like Language Model (NNQLM)~\cite{zhang2018end}. Nonetheless, it is still a traditional neural network with real-valued vectors and density matrices, and therefore insufficient to capture the essential properties of quantum mechanics, as demonstrated in Tab.~\ref{table:Interpretability}. To the best of our knowledge, our study is the first to propose a unified quantum probability framework for fundamental text understanding tasks, with a quantum-inspired formulation and a complex-valued representation for textual data.  

\subsection{Quantum-like Phenomena for Language Understanding}
% \benyou{Any other references about this?}
Quantum-like phenomena in human cognition of information\cite{busemeyer2012quantum,aerts_quantum_2014,aerts_quantum_2004,bruza2008entangling,aerts_concepts_2013}, especially in language understanding, has recently been investigated~\cite{busemeyer2012quantum}. For example,~\citet{bruza2008entangling} discussed word association/entanglement and pointed out that a context might affect word association via the standard interpretation of quantum measurement.~\citet{wang2016exploration} conducted a series of user studies to demonstrate that the document relevance judgment could be largely affected by the previous documents in a quantum-like interference manner. ~\citet{blacoe2013quantum} proposed a bottom-up quantum approach to model distributed semantics with dependency graphs, achieving a competitive performance in word similarity and association tasks. These works provide us with inspirations and insights to investigate in a quantum probabilistic framework to enhance language understanding.


\subsection{Other Quantum-Inspired Approaches}

The discussions on the use of complex numbers have started as early as the advent of quantum-inspired information retrieval (QIR) models. Van Rijsbergen, in his pioneering book of QIR~\cite{van2004geometry}, suggested to use complex numbers as a mechanism to store information, and proposed to assign the amplitude and complex phase to represent TF (Term Frequency) and IDF (Inverse Document Frequency) of a term respectively. This idea was further discussed  in~\citet{zuccon2011use} and implemented on real ad-hoc retrieval datasets. However, it did not achieve better performance than the baseline TF-IDF model.  

Recently, a deep complex network~\cite{trabelsi2017deep} was proposed, where all real layers were replaced with their complex-valued counterparts. Despite the complex-valued structure of the network, the inputs and outputs are real-valued vectors like in any general neural networks, and the model is not related to quantum probability. ~\cite{aerts_towards_2017} elaborated a quantum model for the concepts in a collection of web documents, where a concept admits a complex-valued representation containing an amplitude and a complex phase, and a series of computational methods were developed to model concept combinations and context effects. Only a simple illustrative example was provided, but the model has not been applied to any NLP or IR task. 

\citet{levine2017deep} attempted to draw a connection between quantum entanglement and neural networks, and illustrated that neural networks and quantum mechanics can be more closely connected and integrated. It also motivates us to carry out deeper investigations on this topic in the current and future studies.

\citet{liu2013novel} proposed a novel text classifier based on quantum computation, which tries to find the Hamiltonian matrix and the unitary operator for better fitting the dataset. This model preliminarily reveals the potential of the quantum classifier in supervised learning tasks.


%\section{Preliminary}
%\subsection{From classical probability to quantum probability}

